Deploying ADVISER: Impact and Lessons from Using Artificial Intelligence for Child Vaccination Uptake in Nigeria

More than 5 million children under five years die from largely preventable or treatable medical conditions every year, with an overwhelmingly large proportion of deaths occurring in underdeveloped countries with low vaccination uptake. One of the United Nations' sustainable development goals (SDG 3) aims to end preventable deaths of newborns and children under five years of age. We focus on Nigeria, where the rate of infant mortality is appalling. In particular, low vaccination uptake in Nigeria is a major driver of more than 2,000 daily deaths of children under the age of five years. In this paper, we describe our collaboration with government partners in Nigeria to deploy ADVISER: AI-Driven Vaccination Intervention Optimiser. The framework, based on an integer linear program that seeks to maximize the cumulative probability of successful vaccination, is the first successful deployment of an AI-enabled toolchain for optimizing the allocation of health interventions in Nigeria. In this paper, we provide a background of the ADVISER framework and present results, lessons, and success stories of deploying ADVISER to more than 13,000 families in the state of Oyo, Nigeria.

==> Tables/lessons.tex <==

\begin{table*}[h!]
\resizebox{\textwidth}{!}{\begin{tabular}{lllll}
\hline
\multicolumn{1}{l|}{Intervention}                          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Approx.\\ Model \\ Cost\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Challenges Faced while \\ Designing ADVISER\end{tabular}}                                                                                                                  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Approx.\\ Corrected \\ Cost\end{tabular}} & \multicolumn{1}{c}{Lessons from Deployment}                                                                                                                                                                                                                                                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Phone \\ Calls\end{tabular}     & \$0.4                                                                                & \begin{tabular}[c]{@{}l@{}}We anticipated this to be easiest \\ intervention to administer, based \\ on our prior experience with using\\ phone calls for reminders.\end{tabular}                                         & \$1--2                                                                                   & \begin{tabular}[c]{@{}l@{}}1) Often, cell phones are shared within a family, \\ and mothers are not available when called.\\  2) Moreover, often, multiple calls are required\\ for raising awareness about vaccinations, \\ increasing the cost of intervention per beneficiary.\end{tabular}                                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}Travel \\ Vouchers\end{tabular} & \$1.1                                                                                & \begin{tabular}[c]{@{}l@{}}Travel vouchers do not guarantee\\ success as the vouchers/cash could\\ be used for other trips.\end{tabular}                                                                                  & \$1.1                                                                                    & \begin{tabular}[c]{@{}l@{}}1) We had planned to distribute vouchers for \\ specific carriers and modes, but community\\ discussions highlighted that people preferred\\ different modes (e.g., bus, tricycle, or taxi).\\ 2) Interestingly, we found that our anticipated\\ voucher of \$1.1 per vaccination worked well.\end{tabular}                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}Vaccine\\ Drives\end{tabular}   & \$15                                                                                 & \begin{tabular}[c]{@{}l@{}}A major bottleneck involves buy-in\\ from the state health centers as \\ vaccines must be procured through\\ the state and administered by trained\\ and trusted nurses/midwives.\end{tabular} & \$20                                                                                     & \begin{tabular}[c]{@{}l@{}}1) Our cost of door-to-door vaccination increased\\ due to steep increase in labor (driver) costs, fuel \\ costs, and stipend considerations. \\ 2) Our initial deployment also led to wastage in\\ resources as the cold-box used for door-to-door\\ drives could only maintain the requisite temper-\\ -ature for 2-3 hours.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Pickup \\ Service\end{tabular}  & \$20                                                                                 & \begin{tabular}[c]{@{}l@{}}The major bottleneck we anticipated\\ was the availability of drivers, \\ vehicles, and long waiting times at\\ the health centers.\end{tabular}                                               & \$30                                                                                     & \begin{tabular}[c]{@{}l@{}}1) Our cost for the pickup service increased due\\ to steep increase in labor (driver) and fuel costs.\end{tabular}                                                                                                                                                                                                                         \\ \hline
\end{tabular}}
\caption{Design Challenges and Cost Corrections based on deploying ADVISER.}
\label{tab:challenges}
\end{table*}


==> efficacy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h!]
\centering
\begin{tabular}{@{}lll@{}}
\toprule
Method   & Cumulative Success & Timeline       \\ \midrule
Baseline & 43.6\%             & Aug--Dec 2022  \\
ADVISER  & \textbf{73.9\%}             & Jan--June 2023 \\ \bottomrule
\end{tabular}
\caption{The percentage of beneficiaries whose children received immunization. The ADVISER framework significantly outperformed the baseline during our deployment.}
\label{tab:efficacy}
\end{table}

==> immunizatio_list.tex <==
\begin{table}[h!]
\begin{tabular}{@{}ll@{}}
\toprule
Age                  & Vaccine                                                                                          \\ \midrule
At Birth             & BCG, HEP B, OPV O                                                                                \\
6 Weeks              & PENT 1, PCV 1, OPV 1                                                                             \\
10 Weeks             & PENT 2, PCV 2, OPV 3                                                                             \\
14 Weeks             & PENT 3, PCV 3, OPV 3, IPT                                                                        \\
6 Months             & VIT A 100 Units                                                                                  \\
9 Months             & \begin{tabular}[c]{@{}l@{}}Measles 1, Yellow Fever, \\ Meningitis\end{tabular}                   \\
12 Months            & VIT A RED 200 Units                                                                              \\
15 Months            & Measles 2                                                                                        \\
18 Months to 5 Years & \begin{tabular}[c]{@{}l@{}}VIT A is administered every 6\\  months in this duration\end{tabular} \\ \bottomrule
\end{tabular}
\caption{List of vaccinations tracked by the ADVISER framework. For each does, we typically follow a time window of 7-10 days centered around the prescribed date of the vaccine. Interventions must be matched within these time windows.}
\label{tab:immunization_list}
\end{table}

==> main_AAAI.tex <==
% %File: formatting-instructions-latex-2024.tex
% %release 2024.0
% \documentclass[letterpaper]{article} % DO NOT CHANGE THIS
% \usepackage{aaai24}  % DO NOT CHANGE THIS
% \usepackage{times}  % DO NOT CHANGE THIS
% \usepackage{helvet}  % DO NOT CHANGE THIS
% \usepackage{courier}  % DO NOT CHANGE THIS
% \usepackage[hyphens]{url}  % DO NOT CHANGE THIS
% \usepackage{graphicx} % DO NOT CHANGE THIS
% \urlstyle{rm} % DO NOT CHANGE THIS
% \def\UrlFont{\rm}  % DO NOT CHANGE THIS
% \usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
% \usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
% \frenchspacing  % DO NOT CHANGE THIS
% \setlength{\pdfpagewidth}{8.5in}  % DO NOT CHANGE THIS
% \setlength{\pdfpageheight}{11in}  % DO NOT CHANGE THIS
% %
% % These are recommended to typeset algorithms but not required. See the subsubsection on algorithms. Remove them if you don't have algorithms in your paper.
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{cleveref}
% \usepackage{xcolor}
% \usepackage{booktabs}
% \usepackage{subfigure}
% \usepackage{enumitem}

% %
% % These are are recommended to typeset listings but not required. See the subsubsection on listing. Remove this block if you don't have listings in your paper.
% \usepackage{newfloat}
% \usepackage{listings}
% \DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
% \lstset{%
% 	basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
% 	numbers=left,numberstyle=\footnotesize,xleftmargin=2em,% show line numbers, remove this entire line if you don't want the numbers.
% 	aboveskip=0pt,belowskip=0pt,%
% 	showstringspaces=false,tabsize=2,breaklines=true}
% \floatstyle{ruled}
% \newfloat{listing}{tb}{lst}{}
% \floatname{listing}{Listing}
% %
% % Keep the \pdfinfo as shown here. There's no need
% % for you to add the /Title and /Author tags.
% \pdfinfo{
% /TemplateVersion (2024.1)
% }

% % DISALLOWED PACKAGES
% % \usepackage{authblk} -- This package is specifically forbidden
% % \usepackage{balance} -- This package is specifically forbidden
% % \usepackage{color (if used in text)
% % \usepackage{CJK} -- This package is specifically forbidden
% % \usepackage{float} -- This package is specifically forbidden
% % \usepackage{flushend} -- This package is specifically forbidden
% % \usepackage{fontenc} -- This package is specifically forbidden
% % \usepackage{fullpage} -- This package is specifically forbidden
% % \usepackage{geometry} -- This package is specifically forbidden
% % \usepackage{grffile} -- This package is specifically forbidden
% % \usepackage{hyperref} -- This package is specifically forbidden
% % \usepackage{navigator} -- This package is specifically forbidden
% % (or any other package that embeds links such as navigator or hyperref)
% % \indentfirst} -- This package is specifically forbidden
% % \layout} -- This package is specifically forbidden
% % \multicol} -- This package is specifically forbidden
% % \nameref} -- This package is specifically forbidden
% % \usepackage{savetrees} -- This package is specifically forbidden
% % \usepackage{setspace} -- This package is specifically forbidden
% % \usepackage{stfloats} -- This package is specifically forbidden
% % \usepackage{tabu} -- This package is specifically forbidden
% % \usepackage{titlesec} -- This package is specifically forbidden
% % \usepackage{tocbibind} -- This package is specifically forbidden
% % \usepackage{ulem} -- This package is specifically forbidden
% % \usepackage{wrapfig} -- This package is specifically forbidden
% % DISALLOWED COMMANDS
% % \nocopyright -- Your paper will not be published if you use this command
% % \addtolength -- This command may not be used
% % \balance -- This command may not be used
% % \baselinestretch -- Your paper will not be published if you use this command
% % \clearpage -- No page breaks of any kind may be used for the final version of your paper
% % \columnsep -- This command may not be used
% % \newpage -- No page breaks of any kind may be used for the final version of your paper
% % \pagebreak -- No page breaks of any kind may be used for the final version of your paperr
% % \pagestyle -- This command may not be used
% % \tiny -- This is not an acceptable font size.
% % \vspace{- -- No negative value may be used in proximity of a caption, figure, table, section, subsection, subsubsection, or reference
% % \vskip{- -- No negative value may be used to alter spacing above or below a caption, figure, table, section, subsection, subsubsection, or reference

% \setcounter{secnumdepth}{0} %May be changed to 1 or 2 if section numbers are desired.

% % The file aaai24.sty is the style file for AAAI Press
% % proceedings, working notes, and technical reports.
% %

% % Title

% % Your title must be in mixed case, not sentence case.
% % That means all verbs (including short verbs like be, is, using,and go),
% % nouns, adverbs, adjectives should be capitalized, including both words in hyphenated terms, while
% % articles, conjunctions, and prepositions are lower case unless they
% % directly follow a colon or long dash
% \title{Deploying ADVISER: Impact and Lessons from Using Artificial Intelligence for Child Vaccination Uptake in Nigeria}
% \author{
%     %Authors
%     % All authors must be in the same font size and format.
%     Opadele Kehinde\textsuperscript{\rm 1}, Ruth Abdul\textsuperscript{\rm 1}, Bose Afolabi\textsuperscript{\rm 1}, Parminder Vir\textsuperscript{\rm 1}\\
%     Corinne Namblard\textsuperscript{\rm 1}, Ayan Mukhopadhyay\textsuperscript{\rm 2}\thanks{ayan.mukhopadhyay@vanderbilt.edu}, Abiodun Adereni\thanks{biodun@helpmum.org}\textsuperscript{\rm 1}\\
% }
% \affiliations{
%     %Afiliations
%     \textsuperscript{\rm 1}HelpMum, Ibadan, Nigeria\\
%     \textsuperscript{\rm 2}Vanderbilt University, Nashville, USA\\    
%     % If you have multiple authors and multiple affiliations
%     % use superscripts in text and roman font to identify them.
%     % For example,

%     % Sunil Issar\textsuperscript{\rm 2}, 
%     % J. Scott Penberthy\textsuperscript{\rm 3}, 
%     % George Ferguson\textsuperscript{\rm 4},
%     % Hans Guesgen\textsuperscript{\rm 5}
%     % Note that the comma should be placed after the superscript
%     % 1900 Embarcadero Road, Suite 101\\
%     % Palo Alto, California 94303-3310 USA\\
%     % % email address must be in roman text type, not monospace or sans serif
%     % proceedings-questions@aaai.org
% %
% % See more examples next
% }

% %Example, Single Author, ->> remove \iffalse,\fi and place them surrounding AAAI title to use it
% \iffalse
% \title{My Publication Title --- Single Author}
% \author {
%     Author Name
% }
% \affiliations{
%     Affiliation\\
%     Affiliation Line 2\\
%     name@example.com
% }
% \fi

% \iffalse
% %Example, Multiple Authors, ->> remove \iffalse,\fi and place them surrounding AAAI title to use it
% \title{My Publication Title --- Multiple Authors}
% \author {
%     % Authors
%     First Author Name\textsuperscript{\rm 1,\rm 2},
%     Second Author Name\textsuperscript{\rm 2},
%     Third Author Name\textsuperscript{\rm 1}
% }
% \affiliations {
%     % Affiliations
%     \textsuperscript{\rm 1}Affiliation 1\\
%     \textsuperscript{\rm 2}Affiliation 2\\
%     firstAuthor@affiliation1.com, secondAuthor@affilation2.com, thirdAuthor@affiliation1.com
% }
% \fi


% % REMOVE THIS: bibentry
% % This is only needed to show inline citations in the guidelines document. You should not need it and can safely delete it.
% \usepackage{bibentry}
% % END REMOVE bibentry

% \begin{document}

% \maketitle

% \maketitle
% \input{abstract}
% \input{introduction}
% \input{background}
% \input{deployment}
% \input{results}
% \input{lessons}
% \input{related}
% \input{conclusion}


% \bibliography{aaai24}

% \end{document}

